Out-of-Distribution Detection in Heterogeneous Graphs via Energy Propagation

Graph neural networks (GNNs) are proven effective in extracting complex node and structural information from graph data. While current GNNs perform well in node classification tasks within in-distribution (ID) settings, real-world scenarios often present distribution shifts, leading to the presence of out-of-distribution (OOD) nodes. OOD detection in graphs is a crucial and challenging task. Most existing research focuses on homogeneous graphs, but real-world graphs are often heterogeneous, consisting of diverse node and edge types. This heterogeneity adds complexity and enriches the informational content. To the best of our knowledge, OOD detection in heterogeneous graphs remains an underexplored area. In this context, we propose a novel methodology for OOD detection in heterogeneous graphs (OODHG) that aims to achieve two main objectives: 1) detecting OOD nodes and 2) classifying all ID nodes based on the first task's results. Specifically, we learn representations for each node in the heterogeneous graph, calculate energy values to determine whether nodes are OOD, and then classify ID nodes. To leverage the structural information of heterogeneous graphs, we introduce a meta-path-based energy propagation mechanism and an energy constraint to enhance the distinction between ID and OOD nodes. Extensive experimental findings substantiate the simplicity and effectiveness of OODHG, demonstrating its superiority over baseline models in OOD detection tasks and its accuracy in ID node classification.

==> introduction.tex <==
The rapid progression of graph neural networks (GNNs) has profoundly impacted various domains, where graph data play a crucial role. By extracting rich graph structure information, GNNs have demonstrated a strong ability to model the complex and intricate relationships inherent in graph data~\cite{GraphStructure}. This capability has driven their widespread adoption across a diverse range of domains, including social networks, knowledge graphs, the world wide web, and numerous others. Notably, GNNs offer significant advantages in critical tasks such as node classification~\cite{GCN}, link prediction~\cite{zhang2018link}, and graph classification~\cite{GIN}, providing innovative solutions to long-standing challenges in these fields.

\begin{figure}[!tbp]
  \centering
  \includegraphics[width=\linewidth]{introduction.pdf}
  \caption{An illustration of OOD detection in heterogeneous graphs. The target nodes are authors, and during the training stage, we only utilize a subset of nodes from the ID classes (ID Class1 and ID Class2, as depicted in the figure). The task involves two main objectives: 1) detecting OOD nodes, and 2) classifying ID nodes.
 }
  \label{fig:1}
  \vspace{-3mm}
\end{figure} 

Despite the remarkable achievements of GNNs in numerous applications, a critical limitation remains: most existing research assumes that the training and test data originate from a common distribution~\cite{OpenSet}. Nevertheless, this assumption frequently does not hold in the real-world, where data frequently include out-of-distribution (OOD) samples~\cite{OODSurvey}. OOD samples are data points that deviate from the distribution of the training data, exhibiting discrepancies in features or labels. These samples can severely degrade model performance, resulting in unreliable predictions and impeding robust learning. Addressing this challenge is imperative for enhancing the generalization capability and reliability of GNN-based systems. While significant progress has been made in the areas of OOD generalization~\cite{survey3} and OOD detection~\cite{survey2}, these efforts have predominantly concentrated on image data, which are structured in regular, grid-like forms. In contrast, graph data are inherently irregular and non-Euclidean, consisting of interconnected nodes and edges that encode more complex and often non-linear relationships. This fundamental structural difference necessitates the development of novel, specialised methods that are tailored to the unique properties of graphs. Existing OOD detection techniques, which are well-suited for grid-based image data, are inapplicable to graph-based tasks because of the irregularity and complexity of graph structures.

In recent years, several researchers have started investigating the detection of OOD samples in graphs, with a primary focus on homogeneous graphs. By leveraging message-passing mechanisms to extract structural information from homogeneous graphs, promising results have been achieved in OOD detection~\cite{EMP}. However, real-world graphs are often heterogeneous~\cite{survey}. As graph data continues to be applied across diverse fields, such as social networks~\cite{social,social2}, recommendation systems~\cite{recommend,recommend2}, and citation networks~\cite{GraphSAGE,SimpleHGNN}, the heterogeneity of such data becomes increasingly prominent. In social networks, for instance, users may connect to various interest nodes, resulting in different types of edges. In recommendation systems, the relationships between users and items can take multiple forms, including purchases, views, and ratings. Similarly, in citation networks, nodes correspond to various elements such as authors, papers, and conferences, while edges denote relationships like authorship, citations, and publications. This diversity in node and edge types constructs a heterogeneous graph, which requires managing these varied types and preserving the interaction information between them~\cite{HGNN}—a challenge absent in homogeneous graphs. The additional complexity renders OOD detection methods developed for homogeneous graphs inapplicable to heterogeneous graph settings. In conclusion, conducting OOD detection in heterogeneous graphs is both more challenging and of greater practical significance. Figure \ref{fig:1} illustrates a real-world example of OOD detection in a heterogeneous graph. 

As we know, there is limited research that directly addresses the issue of OOD detection in heterogeneous graphs. Existing methodologies are predominantly devised for homogeneous graphs, overlooking the rich structural information provided by the diverse node and edge types in heterogeneous graphs. This oversight reduces the effectiveness of these methods in practical applications, as real-world graph data is seldom homogeneous. This has led an urgent need for novel approaches capable of accurately detecting OOD samples in heterogeneous graphs. These approaches should account for the unique interactions between various node and edge types, enabling more reliable and effective detection in real-world scenarios.

In this paper, we propose a novel method for OOD detection in heterogeneous graphs (OODHG). The fundamental concept of our approach is to utilize energy scores to identify OOD nodes. Specifically, we first employ heterogeneous graph neural networks (HGNNs) to learn node representations. Subsequently, we compute the energy score for each node based on the logits produced by a multi-layer perceptron (MLP) layer. To fully exploit the structural information inherent in heterogeneous graphs, we introduce a meta-path-based mechanism to propagate energy scores across nodes, refining each node's energy score to more effectively differentiate OOD nodes from ID nodes. Finally, OOD nodes are distinguished from ID nodes based on their energy scores, and ID nodes are classified using softmax probabilities.

To assess the efficacy of the proposed methodology, extensive experiments were conducted on three widely used heterogeneous graph datasets. The experimental results indicate that our method significantly outperforms existing baselines in OOD detection tasks in heterogeneous graphs. In particular, our approach achieves superior performance in both OOD detection and ID classification, demonstrating its robustness and practical relevance in real-world scenarios. This study not only provides a novel perspective on OOD detection in heterogeneous graphs but also lays the foundation for future research in this domain.

Our contributions can be summarized as follows:
\begin{itemize} 
\item To the best of our knowledge, this work represents one of the first systematic attempts to define the problem of OOD detection in heterogeneous graphs.
\item We propose a novel approach that integrates energy scores with the structural information of heterogeneous graphs. Through a meta-path-based energy propagation mechanism, our method efficiently detects OOD nodes. This approach leverages not only the node feature but also the rich structural properties of heterogeneous graphs. 
\item Extensive experiments on multiple heterogeneous graph datasets have been performed to demonstrate the effectiveness and wide applicability of the proposed methodology. \end{itemize}

==> introduction_revised.tex <==
The rapid progression of graph neural networks (GNNs) has profoundly impacted various domains, where graph data play a crucial role. By extracting rich graph structure information, GNNs have demonstrated a strong ability to model the complex and intricate relationships inherent in graph data~\cite{GraphStructure}. This capability has driven their widespread adoption across a diverse range of domains, including social networks, knowledge graphs, the world wide web, and numerous others. Notably, GNNs offer significant advantages in critical tasks such as node classification~\cite{GCN}, link prediction~\cite{zhang2018link}, and graph classification~\cite{GIN}, providing innovative solutions to long-standing challenges in these fields.

\begin{figure}[!tbp]
  \centering
  \includegraphics[width=\linewidth]{introduction.pdf}
  \caption{An illustration of OOD detection in heterogeneous graphs. The target nodes are authors, and during the training stage, we only utilize a subset of nodes from the ID classes (ID Class1 and ID Class2, as depicted in the figure). The task involves two main objectives: 1) detecting OOD nodes, and 2) classifying ID nodes.
 }
  \label{fig:1}
  \vspace{-3mm}
\end{figure} 

Despite the remarkable achievements of GNNs in numerous applications, a critical limitation remains: most existing research assumes that the training and test data originate from a common distribution~\cite{OpenSet}. Nevertheless, this assumption frequently does not hold in the real-world, where data frequently include out-of-distribution (OOD) samples~\cite{OODSurvey}. OOD samples are data points that deviate from the distribution of the training data, exhibiting discrepancies in features or labels. These samples can severely degrade model performance, resulting in unreliable predictions and impeding robust learning. Addressing this challenge is imperative for enhancing the generalization capability and reliability of GNN-based systems. While significant progress has been made in the areas of OOD generalization~\cite{survey3} and OOD detection~\cite{survey2}, these efforts have predominantly concentrated on image data, which are structured in regular, grid-like forms. In contrast, graph data are inherently irregular and non-Euclidean, consisting of interconnected nodes and edges that encode more complex and often non-linear relationships. This fundamental structural difference necessitates the development of novel, specialised methods that are tailored to the unique properties of graphs. Existing OOD detection techniques, which are well-suited for grid-based image data, are inapplicable to graph-based tasks because of the irregularity and complexity of graph structures.

In recent years, several researchers have started investigating the detection of OOD samples in graphs, with a primary focus on homogeneous graphs. By leveraging message-passing mechanisms to extract structural information from homogeneous graphs, promising results have been achieved in OOD detection~\cite{EMP}. However, real-world graphs are often heterogeneous~\cite{survey}. As graph data continues to be applied across diverse fields, such as social networks~\cite{social,social2}, recommendation systems~\cite{recommend,recommend2}, and citation networks~\cite{GraphSAGE,SimpleHGNN}, the heterogeneity of such data becomes increasingly prominent. In social networks, for instance, users may connect to various interest nodes, resulting in different types of edges. In recommendation systems, the relationships between users and items can take multiple forms, including purchases, views, and ratings. Similarly, in citation networks, nodes correspond to various elements such as authors, papers, and conferences, while edges denote relationships like authorship, citations, and publications. This diversity in node and edge types constructs a heterogeneous graph, which requires managing these varied types and preserving the interaction information between them~\cite{HGNN}—a challenge absent in homogeneous graphs. The additional complexity renders OOD detection methods developed for homogeneous graphs inapplicable to heterogeneous graph settings. In conclusion, conducting OOD detection in heterogeneous graphs is both more challenging and of greater practical significance. Figure \ref{fig:1} illustrates a real-world example of OOD detection in a heterogeneous graph. 

As we know, there is limited research that directly addresses the issue of OOD detection in heterogeneous graphs. Existing methodologies are predominantly devised for homogeneous graphs~\cite{OODGAT, GNNSafe}, overlooking the rich structural information provided by the diverse node and edge types in heterogeneous graphs. When applied to heterogeneous graphs, homogeneous graph message-passing mechanisms often focus only on a single type of node, making it difficult to fully capture the complex relationships between different node and edge types. This leads to incomplete information propagation or the loss of critical node information. Such limitations significantly reduce the effectiveness of these methods in practical applications, as real-world graph data is inherently heterogeneous and rarely homogeneous. This has led an urgent need for novel approaches capable of accurately detecting OOD samples in heterogeneous graphs. These approaches should account for the unique interactions between various node and edge types, enabling more reliable and effective detection in real-world scenarios.

In this paper, we propose a novel method for OOD detection in heterogeneous graphs (OODHG). Unlike existing OOD detection methods that primarily focus on homogeneous graphs, our approach is specifically designed to capture the complex structural and semantic relationships in heterogeneous graphs. Our method first employs heterogeneous graph neural networks (HGNNs) to learn node representations while preserving multi-type node and edge dependencies. To quantify the likelihood of a node being OOD, we compute an energy score based on the logits produced by a multi-layer perceptron (MLP) layer. A key innovation of our approach lies in the introduction of a meta-path-based energy propagation mechanism, which refines energy scores by aggregating information from structurally and semantically relevant neighbors. This propagation step allows the model to better exploit the heterogeneous graph structure, leading to improved discrimination between OOD and ID nodes. Finally, OOD nodes are identified based on their refined energy scores, while ID nodes are classified using softmax probabilities. Compared to existing methods, our approach introduces a meta-path energy propagation mechanism, effectively addressing the limitations of homogeneous graph message-passing mechanisms when applied to heterogeneous graphs. This ensures that information transmission remains complete and prevents the loss of important node information.


To assess the efficacy of the proposed methodology, extensive experiments were conducted on three widely used heterogeneous graph datasets. The experimental results indicate that our method significantly outperforms existing baselines in OOD detection tasks in heterogeneous graphs. In particular, our approach achieves superior performance in both OOD detection and ID classification, demonstrating its robustness and practical relevance in real-world scenarios. This study not only provides a novel perspective on OOD detection in heterogeneous graphs but also lays the foundation for future research in this domain.

Our contributions can be summarized as follows:
\begin{itemize} 
\item To the best of our knowledge, this work represents one of the first systematic attempts to define and address the problem of OOD detection in heterogeneous graphs.
\item We propose a novel approach that integrates energy scores with the structural information of heterogeneous graphs. Through a meta-path-based energy propagation mechanism, our method efficiently detects OOD nodes. This approach leverages not only the node feature but also the rich structural properties of heterogeneous graphs. 
\item Extensive experiments on multiple heterogeneous graph datasets have been performed to demonstrate the effectiveness and wide applicability of the proposed methodology. \end{itemize}

==> preliminaries.tex <==
In this section, we present the key definitions of heterogeneous graphs and the OOD detection problem within this context.

\begin{definition}[\textbf{Heterogeneous Graph}]
\textnormal{\( \mathcal{G} = \{ \mathcal{V}, \mathcal{E}, \phi, \psi \} \) represents a heterogeneous graph, where \( \mathcal{V} \) denotes the set of nodes and \( \mathcal{E} \) denotes the set of edges. Each node \( v_i \in \mathcal{V} \) is assigned a type\( \phi(v_i) \), while each edge \( e_{ij} \in \mathcal{E} \) is labeled with a type through \( \psi(e_{ij}) \). The types of nodes and edges are captured by the sets \( T_v = \{ \phi(v) : v \in \mathcal{V} \} \) and \( T_e = \{ \psi(e) : e \in \mathcal{E} \} \), respectively. When \( |T_v| = |T_e| = 1 \), the graph simplifies into a standard homogeneous graph. As shown in Figure~\ref{fig:1}, the heterogeneous graph contains different types of nodes: authors, papers, and conferences. There are edges connecting authors to papers and papers to conferences. The target type $t$ for node classification is authors, meaning that only the nodes representing authors are subject to classification.}
\end{definition}

\begin{definition}[\textbf{Meta-path}] 
\textnormal{A meta-path defines a composite relation of multiple edge types~\cite{metapath}, denoted as \( {P} = t_1 \rightarrow t_2 \rightarrow \ldots \rightarrow t_l \) (abbreviated as \( {P} = t_1 \ldots t_l \)), where \( t_i \) represents a node type. For example, as illustrated in Figure~\ref{fig:1}, two authors can be connected through multiple meta-paths, such as author \(\rightarrow\) paper \(\rightarrow\) author, and author \(\rightarrow\) paper \(\rightarrow\) conference \(\rightarrow\) paper \(\rightarrow\) author.}
\end{definition}
\begin{definition}[\textbf{OOD Detection in Heterogeneous Graphs}]
\textnormal{Given a heterogeneous graph \( \mathcal{G} = \{ \mathcal{V}, \mathcal{E}, \phi, \psi \} \) and a target type \( t \), the set of target nodes \( \mathcal{V}_t = \{ v \in \mathcal{V} \mid \phi(v) = t \} \) is partitioned into two disjoint subsets: \( \mathcal{V}_t = \mathcal{V}_t^{\text{train}} \cup \mathcal{V}_t^{\text{test}} \), where \( \mathcal{V}_t^{\text{train}} \) denotes the training node set and \( \mathcal{V}_t^{\text{test}} \) denotes the test node set. Each node \( v_i \in \mathcal{V}_t^{\text{train}} \) is associated with a label \( y_i \in \{ 1, \ldots, K \} \), where \( K \) represents the number of classes. The test set \( \mathcal{V}_t^{\text{test}} \) is further divided into two subsets: \( \mathcal{V}_t^{\text{test}} = \mathcal{V}_t^{\text{id}} \cup \mathcal{V}_t^{\text{ood}} \), where \( \mathcal{V}_t^{\text{id}} \) represents the set of ID nodes, which belong to the same distribution as those in \( \mathcal{V}_t^{\text{train}} \) and \( \mathcal{V}_t^{\text{ood}} \) represents the OOD nodes, which belong to the different distribution as those in \( \mathcal{V}_t^{\text{train}} \). OOD detection in heterogeneous graphs consists of two primary tasks: 1) identifying OOD nodes in \( \mathcal{V}_t^{\text{ood}} \), and 2) classifying the nodes in \( \mathcal{V}_t^{\text{id}} \). As depicted in Figure~\ref{fig:1}, the training set includes only InD nodes, while the goal is to detect OOD nodes in the test set and classify the ID nodes.}
\end{definition}

==> relatedwork.tex <==
\subsection{Heterogeneous Graph Neural Networks}

It has been demonstrated that GNNs can learn node representations by utilizing both the structural and feature-based information of the graph. Examples of such methods include GCN~\cite{GCN}, GAT~\cite{GAT}, and GraphSAGE~\cite{GraphSAGE}. Nevertheless, these techniques are created primarily for homogeneous graphs and exhibit limitations when extended to heterogeneous graphs. In homogeneous graphs, nodes and edges are of a single type. An example of a homogeneous graph is in social networks where nodes denote users and edges denote friendships. In contrast, heterogeneous graphs comprise a multitude of distinct node and edge types. To illustrate, in an academic network, nodes may represent various entities such as authors, papers, conferences, and research fields, while edges denote relationships such as authorship of papers or the association of papers with specific fields. This diversity within heterogeneous graphs encapsulates richer information but also complicates the task of learning effective node representations.

HAN~\cite{HAN} introduces multiple meta-paths to capture distinct semantic information and employs a multi-level attention mechanism, combined with the GAT model, to capture the significance at both the node and semantic levels in heterogeneous graphs. This represents an early effort in addressing the challenges associated with heterogeneous graph analysis. GTN~\cite{GTN} automatically selects the most important meta-paths, transforming the input heterogeneous graph into meaningful meta-path graphs and learning node representations in an end-to-end way. MAGNN~\cite{MAGNN} encodes all information along a meta-path rather than focusing solely on the nodes at its endpoints, thereby addressing the issue of information loss present in HAN. Simple-HGN~\cite{SimpleHGNN} takes a path-free approach, whereby the features of disparate node types are mapped into a shared feature space. It employs a multi-layer GAT structure, combining node features with learnable edge-type embeddings to learn node representations. SeHGNN~\cite{SEHGNN} implements a monolayer structure that expands the receptive field through long meta-paths, while integrating features from multiple paths using a semantic fusion module.

\subsection{OOD Detection in Graphs}

In machine learning, OOD detection plays a crucial role in assuring model reliability and robustness in real-world applications. Extensive research has been conducted in fields such as computer vision and natural language processing, with approaches including MSP~\cite{MSP}, ODIN~\cite{ODIN}, DOC~\cite{DOC}, and Energy~\cite{Energy}. However, OOD detection presents unique challenges in the context of graph data, as graphs have a non-Euclidean structure.

OOD detection in graphs can be separated into two tasks: node-level and graph-level. Graph-level OOD detection treats each graph as a sample, aiming to detect unseen graphs during the testing phase~\cite{graphood,graphood2}. Node-level OOD detection, which is the focus of this paper, treats each node as a sample and aims to detect nodes with unseen labels during the training phase. Wu et al.~\cite{OpemWGL} are pioneers in studying OOD detection on graphs. They introduce class uncertainty loss constraints to make the model more sensitive to unknown classes. Ultimately, they use a probability threshold to distinguish between ID and OOD nodes, providing a straightforward yet effective method for OOD detection on graph. Zhao et al.~\cite{GKDE} and Stadler et al.~\cite{GPN} expand on this by incorporating multiple types of uncertainty drawn from deep learning and evidence/belief theories. By integrating these uncertainties, their method provides a more robust framework for detecting OOD nodes. Song et al.~\cite{OODGAT} focus on the structural aspects of graph data, discovering that inter-class connections between ID and OOD nodes can hinder the accuracy of OOD detection. To address this, they propose an attention mechanism that selectively emphasizes relevant connections between nodes, improving the separation of ID and OOD nodes. Yang et al.~\cite{EMP} and Wu et al.~\cite{GNNSafe} take a different approach by using entropy and energy-based methods, respectively, to measure the probability that a node belongs to an out-of-distribution class. Both works highlight the importance of leveraging graph structural information through propagation mechanisms, which help to improve the discrimination scores by spreading information across connected nodes, making OOD detection more robust.

==> relatedwork_revised.tex <==
\subsection{Heterogeneous Graph Neural Networks}

It has been demonstrated that GNNs can learn node representations by utilizing both the structural and feature-based information of the graph. Examples of such methods include GCN~\cite{GCN}, GAT~\cite{GAT}, and GraphSAGE~\cite{GraphSAGE}. Nevertheless, these techniques are created primarily for homogeneous graphs and exhibit limitations when extended to heterogeneous graphs. In homogeneous graphs, nodes and edges are of a single type. An example of a homogeneous graph is in social networks where nodes denote users and edges denote friendships. In contrast, heterogeneous graphs comprise a multitude of distinct node and edge types. To illustrate, in an academic network, nodes may represent various entities such as authors, papers, conferences, and research fields, while edges denote relationships such as authorship of papers or the association of papers with specific fields. This diversity within heterogeneous graphs encapsulates richer information but also complicates the task of learning effective node representations.

HAN~\cite{HAN} introduces multiple meta-paths to capture distinct semantic information and employs a multi-level attention mechanism, combined with the GAT model, to capture the significance at both the node and semantic levels in heterogeneous graphs. This represents an early effort in addressing the challenges associated with heterogeneous graph analysis. GTN~\cite{GTN} automatically selects the most important meta-paths, transforming the input heterogeneous graph into meaningful meta-path graphs and learning node representations in an end-to-end way. MAGNN~\cite{MAGNN} encodes all information along a meta-path rather than focusing solely on the nodes at its endpoints, thereby addressing the issue of information loss present in HAN. Simple-HGN~\cite{SimpleHGNN} takes a path-free approach, whereby the features of disparate node types are mapped into a shared feature space. It employs a multi-layer GAT structure, combining node features with learnable edge-type embeddings to learn node representations. SeHGNN~\cite{SEHGNN} implements a monolayer structure that expands the receptive field through long meta-paths, while integrating features from multiple paths using a semantic fusion module.

\subsection{OOD Detection in Graphs}

In machine learning, OOD detection plays a crucial role in assuring model reliability and robustness in real-world applications. Extensive research has been conducted in fields such as computer vision and natural language processing, with approaches including MSP~\cite{MSP}, ODIN~\cite{ODIN}, DOC~\cite{DOC}, and Energy~\cite{Energy}. However, OOD detection presents unique challenges in the context of graph data, as none of these methods consider that graphs have non-Euclidean structures.

OOD detection in graphs can be separated into two tasks: node-level and graph-level. Graph-level OOD detection treats each graph as a sample, aiming to detect unseen graphs during the testing phase~\cite{graphood,graphood2}. Node-level OOD detection, which is the focus of this paper, treats each node as a sample and aims to detect nodes with unseen labels during the training phase. Existing methods for node-level OOD detection can be broadly categorized into two groups: uncertainty-based methods and structure-aware methods. 

Uncertainty-based methods: Wu et al.~\cite{OpemWGL} are pioneers in studying OOD detection on graphs. They introduce class uncertainty loss constraints to make the model more sensitive to unknown classes. Ultimately, they use a probability threshold to distinguish between ID and OOD nodes, providing a straightforward yet effective method for OOD detection on graph. Zhao et al.~\cite{GKDE} and Stadler et al.~\cite{GPN} expand on this by incorporating multiple types of uncertainty drawn from deep learning and evidence/belief theories. By integrating these uncertainties, their method provides a more robust framework for detecting OOD nodes.

Structure-aware methods: Song et al.~\cite{OODGAT} focus on the structural aspects of graph data, discovering that inter-class connections between ID and OOD nodes can hinder the accuracy of OOD detection. To address this, they propose an attention mechanism that selectively emphasizes relevant connections between nodes, improving the separation of ID and OOD nodes. Yang et al.~\cite{EMP} and Wu et al.~\cite{GNNSafe} take a different approach by using entropy and energy-based methods, respectively, to measure the probability that a node belongs to an out-of-distribution class. Both works highlight the importance of leveraging graph structural information through propagation mechanisms, which help to improve the discrimination scores by spreading information across connected nodes, making OOD detection more robust.
